FrameExit: Conditional Early Exiting for Efficient Video Recognition

In this paper, we propose a conditional early exiting framework for efficient video recognition. While existing works focus on selecting a subset of salient frames to reduce the computation costs, we propose to use a simple sampling strategy combined with conditional early exiting to enable efficient recognition. Our model automatically learns to process fewer frames for simpler videos and more frames for complex ones. To achieve this, we employ a cascade of gating modules to automatically determine the earliest point in processing where an inference is sufficiently reliable. We generate on-the-fly supervision signals to the gates to provide a dynamic trade-off between accuracy and computational cost. Our proposed model outperforms competing methods on three large-scale video benchmarks. In particular, on ActivityNet1.3 and mini-kinetics, we outperform the state-of-the-art efficient video recognition methods with 1.3$\times$ and 2.1$\times$ less GFLOPs, respectively. Additionally, our method sets a new state of the art for efficient video understanding on the HVU benchmark.

==> Nick_awesome_texts.tex <==



Gating logic associated with each of the intermediate classifiers may be trained to allow such models to automatically determine the earliest point in processing where an inference is sufficiently reliable

trained to infer the complexity of the intermediate model data for an associated intermediate classifiers 

The inferred complexity of the intermediate model data may be used by gate decision element 208 to decide to process the intermediate model data with the associated intermediate classifier.


[0039]	During training, gates may naturally learn to postpone exiting so that the last (or deepest) classifier always generates the model output (e.g., final classifier 114 in FIG. 1) because that may tend to maximize accuracy at the expense of additional processing. However, this sort of training result largely defeats the purpose of the early exiting architecture depicted in 



[0071]	Note that gate 508A does not include two temporally separate inputs because it processes the first frame, and thus there is no preceding frame. As such, the input to gate 508A is directly from feature extraction model 506 as compared to the gate pre-processing components 512 that provide one of the inputs to gates 508B-D.


indicating whether the model architecture has reached to a confident prediction to exit


generate the determination of whether or not to exit processing by the classification model
